Global semantic typing for inductive and coinductive computing

Inductive and coinductive types are commonly construed as ontological (Church-style) types, denoting canonical data-sets such as natural numbers, lists, and streams. For various purposes, notably the study of programs in the context of global semantics, it is preferable to think of types as semantical properties (Curry-style). Intrinsic theories were introduced in the late 1990s to provide a purely logical framework for reasoning about programs and their semantic types. We extend them here to data given by any combination of inductive and coinductive definitions. This approach is of interest because it fits tightly with syntactic, semantic, and proof theoretic fundamentals of formal logic, with potential applications in implicit computational complexity as well as extraction of programs from proofs. We prove a Canonicity Theorem, showing that the global definition of program typing, via the usual (Tarskian) semantics of first-order logic, agrees with their operational semantics in the intended model. Finally, we show that every intrinsic theory is interpretable in a conservative extension of first-order arithmetic. This means that quantification over infinite data objects does not lead, on its own, to proof-theoretic strength beyond that of Peano Arithmetic. Intrinsic theories are perfectly amenable to formulas-as-types Curry-Howard morphisms, and were used to characterize major computational complexity classes Their extensions described here have similar potential which has already been applied.

==> all.tex <==
% FONTS

\newcommand{\laa}[1]{\begin{CD} @>#1 >> \end{CD}}
	%long annotated arrow, needs package amscd for commuting diagrams
\newcommand{\laaa}[3]{\begin{CD} #1 @>#2 >> #3 \end{CD}}
	%long annotated arrow, including the source and target

\newcommand{\sbnk}{\hbox{\scriptsize $\sqcup$}}
\newcommand{\bnk}{\hbox{\scriptsize $\sqcup$}}

\newcommand{\pfont}{\sffamily\bfseries}
\newcommand{\save}[1]{}

%  SPECIAL CHARACTERS
%  \input{/usr/dml/macros/specialcharacter}
%  \newcommand{\com}{\hbox{`{\Large\bf ,}'}}
% \renewcommand{\leq}{\leqslant}
% \renewcommand{\geq}{\geqslant}
% \newcommand{\lpar}{\hbox{`{\Large\bf (}'}}
% \newcommand{\rpar}{\hbox{`{\Large\bf )}'}}

\newcommand{\id}{\hbox{Id}}
\newcommand{\ffrac}[2]{\hbox{$\frac{#1}{#2}$}}
\newcommand{\proj}{\hbox{${\sf proj}$}}
\newcommand{\trm}{\bxbf{Trm}}
\newcommand{\ctrm}{\bxbf{CTrm}}

\newcommand{\xfig}[2]{\medskip \centerline{\epsfig{figure=#1.eps,height=#2}} \bigskip}

\newcommand{\ul}[1]{\underline{#1}}
\newcommand{\vvec}{\vec}
\newcommand{\binal}{\hbox{$\{\ttzero,\ttone\}$}}	% binary alphabet
\newcommand{\abal}{\hbox{$\{\tta,\ttb\}$}}		% a/b alphabet

\newcommand{\cdlongarrow}[4]{\begin{CD} #1 @>#2 >#3 > #4\end{CD}}

\newcommand{\decar}[1]{\overset{#1}{\Ra}}		% decorated arrow
\newcommand{\arA}[1]{{\stackrel{#1}{\Longrightarrow}}} % annotated right ARROW
\newcommand{\ara}[1]{{\stackrel{#1}{\longrightarrow}}} % annotated right arrow
\newcommand{\uara}[1]{{\underset{#1}{\longrightarrow}}} % under-annotated right arrow
% \newcommand{\uarda}[1]{{\underset{#1}{\twoheadrightarrow}}} % under-annotated double right arrow
\newcommand{\uarda}[1]{{\underset{#1}{\longtwoheadrightarrow}}} % under-annotated double right arrow
\newcommand{\longtwoheadrightarrow}{\longrightarrow\hspace{-1.2em}\rightarrow\hspace{.2em}}
\newcommand{\dara}[2]{\overset{#1}{\underset{#2}{\longrightarrow}}} % doubly annotated right arrow
\newcommand{\ala}[1]{{\stackrel{#1}{\longleftarrow}}} % annotated left arrow
\newcommand{\aara}[2]{{\stackrel{#1}{\longrightarrow}{#2}}} % doubly annotated right arrow
\newcommand{\ldecar}[1]{\overset{#1}{-\!\!\!\Ra}}		% long decorated arrow
\newcommand{\bool}{\hbox{${\cal B}\!\bxit{ool}$}}

\newcommand{\approxsubset}{\raisebox{-.7ex}{$\;\stackrel{\hbox{$\subset$}}{\hbox{\footnotesize$\sim$}}\;$}}

\newcommand{\nmodels}{\,\models\!\!\!\!\!\!/ \;\;}	% not |=

\newcommand{\myred}[1]{\Red{#1}}
\newcommand{\mynicered}[1]{\WildStrawberry{#1}}
% \newcommand{\myred}[1]{\WildStrawberry{#1}}
% \newcommand{\myblue}[1]{\BlueViolet{#1}}
% \newcommand{\myblue}[1]{\Blue{#1}}
% \newcommand{\myblue}[1]{\Violet{#1}}
\newcommand{\myblue}[1]{\RoyalBlue{#1}}
% \newcommand{\mygreen}[1]{\OliveGreen{#1}}
% \newcommand{\mygreen}[1]{\MidnightBlue{#1}}
% \newcommand{\mygreen}[1]{\OliveGreen{#1}}
\newcommand{\mygreen}[1]{\Green{#1}}
\newcommand{\myviolet}[1]{\Violet{#1}}
% \newcommand{\mypurple}[1]{\BlueViolet{#1}}
% \newcommand{\mypurple}[1]{\Violet{#1}}
\newcommand{\mypurple}[1]{\RawSienna{#1}}
\newcommand{\mybrown}[1]{\Mahogany{#1}}
\newcommand{\myorange}[1]{\BurntOrange{#1}}
\newcommand{\mymagenta}[1]{\Magenta{#1}}
\newcommand{\mylime}[1]{\LimeGreen{#1}}
\newcommand{\myblack}[1]{\Black{#1}}
\newcommand{\mywhite}[1]{\White{#1}}
\newcommand{\mygray}[1]{\Gray{#1}}
\newcommand{\mygrey}[1]{\Gray{#1}}

\newcommand{\outt}[1]{}
\newcommand{\delete}[1]{}
\newcommand{\blank}[1]{}
\newcommand{\notedomission}[1]{\medskip\noindent{\bf TEXT OMITTED}\\[2mm]}

\newcommand{\inred}[1]{\hbox{\Red{$#1$}}}
\newcommand{\innicered}[1]{\hbox{\WildStrawberry{$#1$}}}
\newcommand{\inblue}[1]{\hbox{\Blue{$#1$}}}
\newcommand{\ingreen}[1]{\hbox{\OliveGreen{$#1$}}}
\newcommand{\inviolet}[1]{\hbox{\Violet{$#1$}}}
\newcommand{\inbrown}[1]{\hbox{\Mahogany{$#1$}}}
\newcommand{\inorange}[1]{\hbox{\BurtnOrange{$#1$}}}
\newcommand{\inmagenta}[1]{\hbox{\Magenta{$#1$}}}
\newcommand{\inlime}[1]{\hbox{\LimeGreen{$#1$}}}

\newcommand{\cfl}[1]{\begin{array}{c} #1 \end{array}} % centered float in math

\newenvironment{envred}{\textRed}{\textBlack}
\newenvironment{envgray}{\textGray}{\textBlack}
\newenvironment{envblue}{\textBlue}{\textBlack}
\newenvironment{envgreen}{\textOliveGreen}{\textBlack}
\newenvironment{greenenv}{\textOliveGreen}{\textBlack}
\newenvironment{envviolet}{\textViolet}{\textBlack}
\newenvironment{envpurple}{\textPurple}{\textBlack}
\newenvironment{envbrown}{\textMahogany}{\textBlack}
\newenvironment{envorange}{\textBurtnOrange}{\textBlack}
\newenvironment{envmagenta}{\textMagenta}{\textBlack}
\newenvironment{envlime}{\textLimeGreen}{\textBlack}
\newenvironment{envwhite}{\textWhite}{\textBlack}

\newcommand{\bxit}[1]{\hbox{\it #1}}
\newcommand{\bxits}[1]{\hbox{\it #1$\,$}}	%bxit with extra space
\newcommand{\bxitlarge}[1]{\hbox{\large\it #1}}
\newcommand{\bxitLarge}[1]{\hbox{\Large\it #1}}
\newcommand{\bxsf}[1]{\hbox{$\sf #1$}}
\newcommand{\bxrm}[1]{\hbox{\rm #1}}
\newcommand{\bxrmlarge}[1]{\hbox{\large\rm #1}}
\newcommand{\bxrmLarge}[1]{\hbox{\Large\rm #1}}
\newcommand{\bxbf}[1]{\hbox{\bf #1}}
\newcommand{\bxbflarge}[1]{\hbox{\large\bf #1}}
\newcommand{\bxbfLarge}[1]{\hbox{\Large\bf #1}}
\newcommand{\bxsflarge}[1]{\hbox{\large\sf #1}}
\newcommand{\bxsfLarge}[1]{\hbox{\Large\sf #1}}
\newcommand{\bxss}[1]{\hbox{\ss #1}}
\newcommand{\bxsc}[1]{\hbox{\sc #1}}
\newcommand{\bxtt}[1]{\hbox{$\tt #1$}}
\newcommand{\bxttLarge}[1]{\hbox{\Large\tt #1}}
\newcommand{\bxsl}[1]{\hbox{\sl #1}}
\newcommand{\fnbf}[1]{\hbox{\footnotesize\bf #1}}
\newcommand{\fnit}[1]{\hbox{\footnotesize\it #1}}
\newcommand{\fnss}[1]{\hbox{\footnotesize\ss #1}}
\newcommand{\fnsc}[1]{\hbox{\footnotesize\sc #1}}
\newcommand{\fnrm}[1]{\hbox{\footnotesize #1}}
\newcommand{\fntt}[1]{\hbox{\footnotesize\tt #1}}
\newcommand{\fnsl}[1]{\hbox{\footnotesize\sl #1}}
\newcommand{\fnpf}[1]{\hbox{\footnotesize\pfont #1}}
\newcommand{\bfscript}[1]{\hbox{\scriptsize\bf #1}}
\newcommand{\ttscript}[1]{\hbox{\scriptsize\bf #1}}
\newcommand{\sfscript}[1]{\hbox{\scriptsize\sf #1}}
\newcommand{\scriptsf}[1]{\hbox{\scriptsize\sf #1}}
\newcommand{\rmscript}[1]{\hbox{\scriptsize\rm #1}}
\newcommand{\scriptit}[1]{\hbox{\scriptsize\it #1}}
\newcommand{\scriptbf}[1]{\hbox{\scriptsize\bf #1}}
\newcommand{\scripttt}[1]{\hbox{\scriptsize\bf #1}}
\newcommand{\scriptrm}[1]{\hbox{\scriptsize\rm #1}}
\newcommand{\itscript}[1]{\hbox{\scriptsize\it #1}}
\newcommand{\scscript}[1]{\hbox{\scriptsize\sc #1}}
\newcommand{\scriptsc}[1]{\hbox{\scriptsize\sc #1}}
\newcommand{\smallrm}[1]{\hbox{\small\rm #1}}
\newcommand{\smallit}[1]{\hbox{\small\it #1}}
\newcommand{\smallbf}[1]{\hbox{\small\bf #1}}
\newcommand{\smalltt}[1]{\hbox{\small\tt #1}}
\newcommand{\smallsl}[1]{\hbox{\small\sl #1}}
\newcommand{\smallsf}[1]{\hbox{\small\sf #1}}
\newcommand{\bxpf}[1]{\smallsf{#1}}
\newcommand{\largerm}[1]{\hbox{\large\rm #1}}
\newcommand{\Largerm}[1]{\hbox{\Large\rm #1}}
\newcommand{\Largepf}[1]{\hbox{\Large\pfont #1}}
\newcommand{\largepf}[1]{\hbox{\large\pfont #1}}
\newcommand{\largeit}[1]{\hbox{\large\it #1}}
\newcommand{\Largeit}[1]{\hbox{\large\it #1}}
\newcommand{\largebf}[1]{\hbox{\large\bf #1}}
\newcommand{\Largebf}[1]{\hbox{\Large\bf #1}}
\newcommand{\largett}[1]{\hbox{\large\tt #1}}
\newcommand{\largesl}[1]{\hbox{\large\sl #1}}
\newcommand{\fnc}[1]{\mbox{\underline{\it #1}$\,$}}
\newcommand{\mfnc}[1]{\mbox{\underline{\rm #1}$\,$}} % meta-functions
\newcommand{\ident}[1]{\mbox{\underline{\sf #1}$\,$}}

\newcommand{\mathl}{\hbox{$\ell$}}

\newcommand{\bfa}{{\bf a}}
\newcommand{\bfb}{{\bf b}}
\newcommand{\bfc}{{\bf c}}
\newcommand{\bfd}{{\bf d}}
\newcommand{\bfe}{{\bf e}}
\newcommand{\bff}{{\bf f}}
\newcommand{\bfg}{{\bf g}}
\newcommand{\bfh}{{\bf h}}
\newcommand{\bfi}{{\bf i}}
\newcommand{\bfj}{{\bf j}}
\newcommand{\bfk}{{\bf k}}
\newcommand{\bfl}{{\bf l}}
\newcommand{\bfm}{{\bf m}}
\newcommand{\bfn}{{\bf n}}
\newcommand{\bfo}{{\bf o}}
\newcommand{\bfp}{{\bf p}}
\newcommand{\bfq}{{\bf q}}
\newcommand{\bfr}{{\bf r}}
\newcommand{\bfs}{{\bf s}}
\newcommand{\bft}{{\bf t}}
\newcommand{\bfu}{{\bf u}}
\newcommand{\bfv}{{\bf v}}
\newcommand{\bfw}{{\bf w}}
\newcommand{\bfx}{{\bf x}}
\newcommand{\bfy}{{\bf y}}
\newcommand{\bfz}{{\bf z}}

\newcommand{\ita}{{\it a}}
\newcommand{\itb}{{\it b}}
\newcommand{\itc}{{\it c}}
\newcommand{\itd}{{\it d}}
\newcommand{\ite}{{\it e}}
\newcommand{\itf}{{\it f}}
\newcommand{\itg}{{\it g}}
\newcommand{\ith}{{\it h}}
\newcommand{\iti}{{\it i}}
\newcommand{\itj}{{\it j}}
\newcommand{\itk}{{\it k}}
\newcommand{\itl}{{\it l}}
\newcommand{\itm}{{\it m}}
\newcommand{\itn}{{\it n}}
\newcommand{\ito}{{\it o}}
\newcommand{\itp}{{\it p}}
\newcommand{\itq}{{\it q}}
\newcommand{\itr}{{\it r}}
\newcommand{\its}{{\it s}}
\newcommand{\itt}{{\it t}}
\newcommand{\itu}{{\it u}}
\newcommand{\itv}{{\it v}}
\newcommand{\itw}{{\it w}}
\newcommand{\itx}{{\it x}}
\newcommand{\ity}{{\it y}}
\newcommand{\itz}{{\it z}}

\newcommand{\sfa}{\bxsf{a}}
\newcommand{\sfb}{\bxsf{b}}
\newcommand{\sfc}{\bxsf{c}}
\newcommand{\sfd}{\bxsf{d}}
\newcommand{\sfe}{\bxsf{e}}
\newcommand{\sff}{\bxsf{f}}
\newcommand{\sfg}{\bxsf{g}}
\newcommand{\sfh}{\bxsf{h}}
\newcommand{\sfi}{\bxsf{i}}
\newcommand{\sfj}{\bxsf{j}}
\newcommand{\sfk}{\bxsf{k}}
\newcommand{\sfl}{\bxsf{l}}
\newcommand{\sfm}{\bxsf{m}}
\newcommand{\sfn}{\bxsf{n}}
\newcommand{\sfo}{\bxsf{o}}
\newcommand{\sfp}{\bxsf{p}}
\newcommand{\sfq}{\bxsf{q}}
\newcommand{\sfr}{\bxsf{r}}
\newcommand{\sfs}{\bxsf{s}}
\newcommand{\sft}{\bxsf{t}}
\newcommand{\sfu}{\bxsf{u}}
\newcommand{\sfv}{\bxsf{v}}
\newcommand{\sfw}{\bxsf{w}}
\newcommand{\sfx}{\bxsf{x}}
\newcommand{\sfy}{\bxsf{y}}
\newcommand{\sfz}{\bxsf{z}}

\newcommand{\sfA}{{\sf A}}
\newcommand{\sfB}{{\sf B}}
\newcommand{\sfC}{{\sf C}}
\newcommand{\sfD}{{\sf D}}
\newcommand{\sfE}{{\sf E}}
\newcommand{\sfF}{{\sf F}}
\newcommand{\sfG}{{\sf G}}
\newcommand{\sfH}{{\sf H}}
\newcommand{\sfI}{{\sf I}}
\newcommand{\sfJ}{{\sf J}}
\newcommand{\sfK}{{\sf K}}
\newcommand{\sfL}{{\sf L}}
\newcommand{\sfM}{{\sf M}}
\newcommand{\sfN}{{\sf N}}
\newcommand{\sfO}{{\sf O}}
\newcommand{\sfP}{{\sf P}}
\newcommand{\sfQ}{{\sf Q}}
\newcommand{\sfR}{{\sf R}}
\newcommand{\sfS}{{\sf S}}
\newcommand{\sfT}{{\sf T}}
\newcommand{\sfU}{{\sf U}}
\newcommand{\sfV}{{\sf V}}
\newcommand{\sfW}{{\sf W}}
\newcommand{\sfX}{{\sf X}}
\newcommand{\sfY}{{\sf Y}}
\newcommand{\sfZ}{{\sf Z}}

\newcommand{\scsfa}{{\scriptsize\sf a}}
\newcommand{\scsfb}{{\scriptsize\sf b}}
\newcommand{\scsfc}{{\scriptsize\sf c}}
\newcommand{\scsfd}{{\scriptsize\sf d}}
\newcommand{\scsfe}{{\scriptsize\sf e}}
\newcommand{\scsff}{{\scriptsize\sf f}}
\newcommand{\scsfg}{{\scriptsize\sf g}}
\newcommand{\scsfh}{{\scriptsize\sf h}}
\newcommand{\scsfi}{{\scriptsize\sf i}}
\newcommand{\scsfj}{{\scriptsize\sf j}}
\newcommand{\scsfk}{{\scriptsize\sf k}}
\newcommand{\scsfl}{{\scriptsize\sf l}}
\newcommand{\scsfm}{{\scriptsize\sf m}}
\newcommand{\scsfn}{{\scriptsize\sf n}}
\newcommand{\scsfo}{{\scriptsize\sf o}}
\newcommand{\scsfp}{{\scriptsize\sf p}}
\newcommand{\scsfq}{{\scriptsize\sf q}}
\newcommand{\scsfr}{{\scriptsize\sf r}}
\newcommand{\scsfs}{{\scriptsize\sf s}}
\newcommand{\scsft}{{\scriptsize\sf t}}
\newcommand{\scsfu}{{\scriptsize\sf u}}
\newcommand{\scsfv}{{\scriptsize\sf v}}
\newcommand{\scsfw}{{\scriptsize\sf w}}
\newcommand{\scsfx}{{\scriptsize\sf x}}
\newcommand{\scsfy}{{\scriptsize\sf y}}
\newcommand{\scsfz}{{\scriptsize\sf z}}

\newcommand{\rma}{{\rm a}}
\newcommand{\rmb}{{\rm b}}
\newcommand{\rmc}{{\rm c}}
\newcommand{\rmd}{{\rm d}}
\newcommand{\rme}{{\rm e}}
\newcommand{\rmf}{{\rm f}}
\newcommand{\rmg}{{\rm g}}
\newcommand{\rmh}{{\rm h}}
\newcommand{\rmi}{{\rm i}}
\newcommand{\rmj}{{\rm j}}
\newcommand{\rmk}{{\rm k}}
\newcommand{\rml}{{\rm l}}
\newcommand{\rmm}{{\rm m}}
\newcommand{\rmn}{{\rm n}}
\newcommand{\rmo}{{\rm o}}
\newcommand{\rmp}{{\rm p}}
\newcommand{\rmq}{{\rm q}}
\newcommand{\rmr}{{\rm r}}
\newcommand{\rms}{{\rm s}}
\newcommand{\rmt}{{\rm t}}
\newcommand{\rmu}{{\rm u}}
\newcommand{\rmv}{{\rm v}}
\newcommand{\rmw}{{\rm w}}
\newcommand{\rmx}{{\rm x}}
\newcommand{\rmy}{{\rm y}}
\newcommand{\rmz}{{\rm z}}
\newcommand{\rmone}{{\rm 1}}
\newcommand{\rmtwo}{{\rm 2}}
\newcommand{\rmthree}{{\rm 3}}
\newcommand{\rmfour}{{\rm 4}}
\newcommand{\rmfive}{{\rm 5}}
\newcommand{\rmsix}{{\rm 6}}
\newcommand{\rmseven}{{\rm 7}}
\newcommand{\rmeight}{{\rm 8}}
\newcommand{\rmnine}{{\rm 9}}
\newcommand{\rmzero}{{\rm 0}}

\newcommand{\tta}{\hbox{$\tt a$}}
\newcommand{\ttb}{\hbox{$\tt b$}}
\newcommand{\ttc}{\hbox{$\tt c$}}
\newcommand{\ttd}{\hbox{$\tt d$}}
\newcommand{\tte}{\hbox{$\tt e$}}
\newcommand{\ttf}{\hbox{$\tt f$}}
\newcommand{\ttg}{\hbox{$\tt g$}}
\newcommand{\tth}{\hbox{$\tt h$}}
\newcommand{\tti}{\hbox{$\tt i$}}
\newcommand{\ttj}{\hbox{$\tt j$}}
\newcommand{\ttk}{\hbox{$\tt k$}}
\newcommand{\ttl}{\hbox{$\tt l$}}
\newcommand{\ttm}{\hbox{$\tt m$}}
\newcommand{\ttn}{\hbox{$\tt n$}}
\newcommand{\tto}{\hbox{$\tt o$}}
\newcommand{\ttp}{\hbox{$\tt p$}}
\newcommand{\ttq}{\hbox{$\tt q$}}
\newcommand{\ttr}{\hbox{$\tt r$}}
\newcommand{\tts}{\hbox{$\tt s$}}
\newcommand{\ttt}{\hbox{$\tt t$}}
\newcommand{\ttu}{\hbox{$\tt u$}}
\newcommand{\ttv}{\hbox{$\tt v$}}
\newcommand{\ttw}{\hbox{$\tt w$}}
\newcommand{\ttx}{\hbox{$\tt x$}}
\newcommand{\uttx}{\hbox{${\tt \underline{x}}$}}
\newcommand{\tty}{\hbox{$\tt y$}}
\newcommand{\ttz}{\hbox{$\tt z$}}
\newcommand{\ttdollar}{\hbox{$\tt \$ $}}
\newcommand{\ttzero}{\hbox{$\tt 0$}}
\newcommand{\uttzero}{\hbox{$\tt \underline{0}}}
\newcommand{\ttone}{\hbox{$\tt 1$}}
\newcommand{\uttone}{\hbox{$\tt \underline{1}$}}
\newcommand{\tttwo}{\hbox{\tt 2}}
\newcommand{\ttthree}{\hbox{\tt 3}}
\newcommand{\ttfour}{\hbox{\tt 4}}
\newcommand{\ttfive}{\hbox{\tt 5}}
\newcommand{\ttsix}{\hbox{\tt 6}}
\newcommand{\ttseven}{\hbox{\tt 7}}
\newcommand{\tteight}{\hbox{\tt 8}}
\newcommand{\ttnine}{\hbox{\tt 9}}
% \newcommand{\ttdollar}{\hbox{\tt \$}}
\newcommand{\ttpound}{\hbox{\pounds}}
\newcommand{\tteqn}{\hbox{\tt =}}

\newcommand{\sca}{\hbox{\sc a}}
\newcommand{\scb}{\hbox{\sc b}}
\newcommand{\scc}{\hbox{\sc c}}
\newcommand{\scd}{\hbox{\sc d}}
\newcommand{\sce}{\hbox{\sc e}}
\newcommand{\scf}{\hbox{\sc f}}
\newcommand{\scg}{\hbox{\sc g}}
\newcommand{\sch}{\hbox{\sc h}}
\newcommand{\sci}{\hbox{\sc i}}
\newcommand{\scj}{\hbox{\sc j}}
\newcommand{\sck}{\hbox{\sc k}}
\newcommand{\scl}{\hbox{\sc l}}
\newcommand{\scm}{\hbox{\sc m}}
\newcommand{\scn}{\hbox{\sc n}}
\newcommand{\sco}{\hbox{\sc o}}
\newcommand{\scp}{\hbox{\sc p}}
\newcommand{\scq}{\hbox{\sc q}}
\newcommand{\scr}{\hbox{\sc r}}
\newcommand{\scs}{\hbox{\sc s}}
\newcommand{\sct}{\hbox{\sc t}}
\newcommand{\scu}{\hbox{\sc u}}
\newcommand{\scv}{\hbox{\sc v}}
\newcommand{\scw}{\hbox{\sc w}}
\newcommand{\scx}{\hbox{\sc x}}
\newcommand{\scy}{\hbox{\sc y}}
\newcommand{\scz}{\hbox{\sc z}}

\newcommand{\bfA}{{\bf A}}
\newcommand{\bfB}{{\bf B}}
\newcommand{\bfC}{{\bf C}}
\newcommand{\bfD}{{\bf D}}
\newcommand{\bfE}{{\bf E}}
\newcommand{\bfF}{{\bf F}}
\newcommand{\bfG}{{\bf G}}
\newcommand{\bfH}{{\bf H}}
\newcommand{\bfI}{{\bf I}}
\newcommand{\bfJ}{{\bf J}}
\newcommand{\bfK}{{\bf K}}
\newcommand{\bfL}{{\bf L}}
\newcommand{\bfM}{{\bf M}}
\newcommand{\bfN}{{\bf N}}
\newcommand{\bfO}{{\bf O}}
\newcommand{\bfP}{{\bf P}}
\newcommand{\bfQ}{{\bf Q}}
\newcommand{\bfR}{{\bf R}}
\newcommand{\bfS}{{\bf S}}
\newcommand{\bfT}{{\bf T}}
\newcommand{\bfU}{{\bf U}}
\newcommand{\bfV}{{\bf V}}
\newcommand{\bfW}{{\bf W}}
\newcommand{\bfX}{{\bf X}}
\newcommand{\bfY}{{\bf Y}}
\newcommand{\bfZ}{{\bf Z}}

\newcommand{\pfa}{\mbox{\small\pfont a}}
\newcommand{\pfb}{\mbox{\small\pfont b}}
\newcommand{\pfc}{\mbox{\small \pfont c}}
\newcommand{\pfd}{\mbox{\small\pfont d}}
\newcommand{\pfe}{\mbox{\small\pfont e}}
\newcommand{\pff}{\mbox{\small\pfont f}}
\newcommand{\pfg}{\mbox{\small\pfont g}}
\newcommand{\pfh}{\mbox{\small\pfont h}}
\newcommand{\pfi}{\mbox{\small\pfont i}}
\newcommand{\pfj}{\mbox{\small\pfont j}}
\newcommand{\pfk}{\mbox{\small\pfont k}}
\newcommand{\pfl}{\mbox{\small\pfont l}}
\newcommand{\pfm}{\mbox{\small\pfont m}}
\newcommand{\pfn}{\mbox{\small\pfont n}}
\newcommand{\pfo}{\mbox{\small\pfont o}}
\newcommand{\pfp}{\mbox{\small\pfont p}}
\newcommand{\pfq}{\mbox{\small\pfont q}}
\newcommand{\pfr}{\mbox{\small\pfont r}}
\newcommand{\pfs}{\mbox{\small\pfont s}}
\newcommand{\pft}{\mbox{\small\pfont t}}
\newcommand{\pfu}{\mbox{\small\pfont u}}
\newcommand{\pfv}{\mbox{\small\pfont v}}
\newcommand{\pfw}{\mbox{\small\pfont w}}
\newcommand{\pfx}{\mbox{\small\pfont x}}
\newcommand{\pfy}{\mbox{\small\pfont y}}
\newcommand{\pfz}{\mbox{\small\pfont z}}

\newcommand{\pfA}{\mbox{\small\pfont A}}
\newcommand{\pfB}{\mbox{\small\pfont B}}
\newcommand{\pfC}{\mbox{\small\pfont C}}
\newcommand{\pfD}{\mbox{\small\pfont D}}
\newcommand{\pfE}{\mbox{\small\pfont E}}
\newcommand{\pfF}{\mbox{\small\pfont F}}
\newcommand{\pfG}{\mbox{\small\pfont G}}
\newcommand{\pfH}{\mbox{\small\pfont H}}
\newcommand{\pfI}{\mbox{\small\pfont I}}
\newcommand{\pfJ}{\mbox{\small\pfont J}}
\newcommand{\pfK}{\mbox{\small\pfont K}}
\newcommand{\pfL}{\mbox{\small\pfont L}}
\newcommand{\pfM}{\mbox{\small\pfont M}}
\newcommand{\pfN}{\mbox{\small\pfont N}}
\newcommand{\pfO}{\mbox{\small\pfont O}}
\newcommand{\pfP}{\mbox{\small\pfont P}}
\newcommand{\pfQ}{\mbox{\small\pfont Q}}
\newcommand{\pfR}{\mbox{\small\pfont R}}
\newcommand{\pfS}{\mbox{\small\pfont S}}
\newcommand{\pfT}{\mbox{\small\pfont T}}
\newcommand{\pfU}{\mbox{\small\pfont U}}
\newcommand{\pfV}{\mbox{\small\pfont V}}
\newcommand{\pfW}{\mbox{\small\pfont W}}
\newcommand{\pfX}{\mbox{\small\pfont X}}
\newcommand{\pfY}{\mbox{\small\pfont Y}}
\newcommand{\pfZ}{\mbox{\small\pfont Z}}

% \newcommand{\sla}{\mbox{\small\sl a}}
% \newcommand{\slb}{\mbox{\small\sl b}}
\newcommand{\slc}{\mbox{\small \sl c}}
\newcommand{\sld}{\mbox{\small\sl d}}
\newcommand{\sle}{\mbox{\small\sl e}}
\newcommand{\slf}{\mbox{\small\sl f}}
\newcommand{\slg}{\mbox{\small\sl g}}
\newcommand{\slh}{\mbox{\small\sl h}}
\newcommand{\sli}{\mbox{\small\sl i}}
\newcommand{\slj}{\mbox{\small\sl j}}
\newcommand{\slk}{\mbox{\small\sl k}}
\newcommand{\sll}{\mbox{\small\sl l}}
\newcommand{\slm}{\mbox{\small\sl m}}
\newcommand{\sln}{\mbox{\small\sl n}}
\newcommand{\slo}{\mbox{\small\sl o}}
\newcommand{\slp}{\mbox{\small\sl p}}
\newcommand{\slq}{\mbox{\small\sl q}}
\newcommand{\slr}{\mbox{\small\sl r}}
\newcommand{\sls}{\mbox{\small\sl s}}
\newcommand{\slt}{\mbox{\small\sl t}}
\newcommand{\slu}{\mbox{\small\sl u}}
\newcommand{\slv}{\mbox{\small\sl v}}
\newcommand{\slw}{\mbox{\small\sl w}}
\newcommand{\slx}{\mbox{\small\sl x}}
\newcommand{\sly}{\mbox{\small\sl y}}
\newcommand{\slz}{\mbox{\small\sl z}}

\newcommand{\slA}{\mbox{\small\sl A}}
\newcommand{\slB}{\mbox{\small\sl B}}
\newcommand{\slC}{\mbox{\small\sl C}}
\newcommand{\slD}{\mbox{\small\sl D}}
\newcommand{\slE}{\mbox{\small\sl E}}
\newcommand{\slF}{\mbox{\small\sl F}}
\newcommand{\slG}{\mbox{\small\sl G}}
\newcommand{\slH}{\mbox{\small\sl H}}
\newcommand{\slI}{\mbox{\small\sl I}}
\newcommand{\slJ}{\mbox{\small\sl J}}
\newcommand{\slK}{\mbox{\small\sl K}}
\newcommand{\slL}{\mbox{\small\sl L}}
\newcommand{\slM}{\mbox{\small\sl M}}
\newcommand{\slN}{\mbox{\small\sl N}}
\newcommand{\slO}{\mbox{\small\sl O}}
\newcommand{\slP}{\mbox{\small\sl P}}
\newcommand{\slQ}{\mbox{\small\sl Q}}
\newcommand{\slR}{\mbox{\small\sl R}}
\newcommand{\slS}{\mbox{\small\sl S}}
\newcommand{\slT}{\mbox{\small\sl T}}
\newcommand{\slU}{\mbox{\small\sl U}}
\newcommand{\slV}{\mbox{\small\sl V}}
\newcommand{\slW}{\mbox{\small\sl W}}
\newcommand{\slX}{\mbox{\small\sl X}}
\newcommand{\slY}{\mbox{\small\sl Y}}
\newcommand{\slZ}{\mbox{\small\sl Z}}

% \emm is for definitions.
\newcommand{\emm}[1]{\fbox{\sl#1}}

% \Idt font is modular, can be changed by redifining \Idt
\newcommand{\Idt}{\sf}
\newcommand{\ida}{\mbox{\underline{\Idt a}}}
\newcommand{\idb}{\mbox{\underline{\Idt b}}}
\newcommand{\idc}{\mbox{\underline{\Idt c}}}
\newcommand{\idd}{\mbox{\underline{\Idt d}}}
\newcommand{\ide}{\mbox{\underline{\Idt e}}}
\newcommand{\idf}{\mbox{\underline{\Idt f}}}
\newcommand{\idg}{\mbox{\underline{\Idt g}}}
\newcommand{\idh}{\mbox{\underline{\Idt h}}}
\newcommand{\idi}{\mbox{\underline{\Idt i}}}
\newcommand{\idj}{\mbox{\underline{\Idt j}}}
\newcommand{\idk}{\mbox{\underline{\Idt k}}}
\newcommand{\idl}{\mbox{\underline{\Idt l}}}
\newcommand{\idm}{\mbox{\underline{\Idt m}}}
\newcommand{\idn}{\mbox{\underline{\Idt n}}}
\newcommand{\ido}{\mbox{\underline{\Idt o}}}
\newcommand{\idp}{\mbox{\underline{\Idt p}}}
\newcommand{\idq}{\mbox{\underline{\Idt q}}}
\newcommand{\idr}{\mbox{\underline{\Idt r}}}
\newcommand{\ids}{\mbox{\underline{\Idt s}}}
\newcommand{\idt}{\mbox{\underline{\Idt t}}}
\newcommand{\idu}{\mbox{\underline{\Idt u}}}
\newcommand{\idv}{\mbox{\underline{\Idt v}}}
\newcommand{\idw}{\mbox{\underline{\Idt w}}}
\newcommand{\idx}{\mbox{\underline{\Idt x}}}
\newcommand{\idy}{\mbox{\underline{\Idt y}}}
\newcommand{\idz}{\mbox{\underline{\Idt z}}}
\newcommand{\idA}{\mbox{\underline{\Idt A}}}
\newcommand{\idB}{\mbox{\underline{\Idt B}}}
\newcommand{\idC}{\mbox{\underline{\Idt C}}}
\newcommand{\idD}{\mbox{\underline{\Idt D}}}
\newcommand{\idE}{\mbox{\underline{\Idt E}}}
\newcommand{\idF}{\mbox{\underline{\Idt F}}}
\newcommand{\idG}{\mbox{\underline{\Idt G}}}
\newcommand{\idH}{\mbox{\underline{\Idt H}}}
\newcommand{\idI}{\mbox{\underline{\Idt I}}}
\newcommand{\idJ}{\mbox{\underline{\Idt J}}}
\newcommand{\idK}{\mbox{\underline{\Idt K}}}
\newcommand{\idL}{\mbox{\underline{\Idt L}}}
\newcommand{\idM}{\mbox{\underline{\Idt M}}}
\newcommand{\idN}{\mbox{\underline{\Idt N}}}
\newcommand{\idO}{\mbox{\underline{\Idt O}}}
\newcommand{\idP}{\mbox{\underline{\Idt P}}}
\newcommand{\idQ}{\mbox{\underline{\Idt Q}}}
\newcommand{\idR}{\mbox{\underline{\Idt R}}}
\newcommand{\idS}{\mbox{\underline{\Idt S}}}
\newcommand{\idT}{\mbox{\underline{\Idt T}}}
\newcommand{\idU}{\mbox{\underline{\Idt U}}}
\newcommand{\idV}{\mbox{\underline{\Idt V}}}
\newcommand{\idW}{\mbox{\underline{\Idt W}}}
\newcommand{\idX}{\mbox{\underline{\Idt X}}}
\newcommand{\idY}{\mbox{\underline{\Idt Y}}}
\newcommand{\idZ}{\mbox{\underline{\Idt Z}}}
\newcommand{\idzero}{\mbox{\underline{\Idt 0}}}
\newcommand{\idone}{\mbox{\underline{\Idt 1}}}
\newcommand{\idtwo}{\mbox{\underline{\Idt 2}}}
\newcommand{\idthree}{\mbox{\underline{\Idt 3}}}
\newcommand{\idfour}{\mbox{\underline{\Idt 4}}}
\newcommand{\idfive}{\mbox{\underline{\Idt 5}}}
\newcommand{\idsix}{\mbox{\underline{\Idt 6}}}
\newcommand{\idseven}{\mbox{\underline{\Idt 7}}}
\newcommand{\ideight}{\mbox{\underline{\Idt 8}}}
\newcommand{\idnine}{\mbox{\underline{\Idt 9}}}
\newcommand{\bxid}[1]{\mbox{\underline{\id #1}}}
%\newcommand{\bxid}[1]{\mbox{\underline{\normalsize\id #1}}}

\newcommand{\idbgra}{\mbox{\underline{\boldmath$\alpha$}}}
\newcommand{\idbgrb}{\mbox{\underline{\boldmath$\beta$}}}
\newcommand{\idbgrg}{\mbox{\underline{\boldmath$\gamma$}}}
\newcommand{\idbgrd}{\mbox{\underline{\boldmath$\delta$}}}
\newcommand{\idbgre}{\mbox{\underline{\boldmath$\varepsilon$}}}
\newcommand{\idbgrz}{\mbox{\underline{\boldmath$\zeta$}}}
\newcommand{\idbgrh}{\mbox{\underline{\boldmath$\eta$}}}
\newcommand{\idbgrth}{\mbox{\underline{\boldmath$\theta$}}}
\newcommand{\idbgri}{\mbox{\underline{\boldmath$\iota$}}}
\newcommand{\idbgrk}{\mbox{\underline{\boldmath$\kappa$}}}
\newcommand{\idbgrl}{\mbox{\underline{\boldmath$\lambda$}}}
\newcommand{\idbgrm}{\mbox{\underline{\boldmath$\mu$}}}
\newcommand{\idbgrn}{\mbox{\underline{\boldmath$\nu$}}}
\newcommand{\idbgrx}{\mbox{\underline{\boldmath$\xi$}}}
\newcommand{\idbgro}{\mbox{\underline{\boldmath$\omicron$}}}
\newcommand{\idbgrp}{\mbox{\underline{\boldmath$\pi$}}}
\newcommand{\idbgrr}{\mbox{\underline{\boldmath$\rho$}}}
\newcommand{\idbgrs}{\mbox{\underline{\boldmath$\sigma$}}}
\newcommand{\idbgrt}{\mbox{\underline{\boldmath$\tau$}}}
\newcommand{\idbgru}{\mbox{\underline{\boldmath$\upsilon$}}}
\newcommand{\idbgrf}{\mbox{\underline{\boldmath$\varphi$}}}
\newcommand{\idbgrch}{\mbox{\underline{\boldmath$\chi$}}}
\newcommand{\idbgrq}{\mbox{\underline{\boldmath$\psi$}}}
\newcommand{\idbgrw}{\mbox{\underline{\boldmath$\omega$}}}

\newcommand{\idbgrG}{\mbox{\underline{\boldmath$\Gamma$}}}
\newcommand{\idbgrD}{\mbox{\underline{\boldmath$\Delta$}}}
\newcommand{\idbgrT}{\mbox{\underline{\boldmath$\Theta$}}}
\newcommand{\idbgrL}{\mbox{\underline{\boldmath$\Lambda$}}}
\newcommand{\idbgrX}{\mbox{\underline{\boldmath$\Xi$}}}
\newcommand{\idbgrP}{\mbox{\underline{\boldmath$\Pi$}}}
\newcommand{\idbgrS}{\mbox{\underline{\boldmath$\Sigma$}}}
\newcommand{\idbgrU}{\mbox{\underline{\boldmath$\Upsilon$}}}
\newcommand{\idbgrF}{\mbox{\underline{\boldmath$\Phi$}}}
\newcommand{\idbgrQ}{\mbox{\underline{\boldmath$\Psi$}}}
\newcommand{\idbgrW}{\mbox{\underline{\boldmath$\Omega$}}}


\newcommand{\bfminus}{\mbox{\bf --}}
\newcommand{\bfzero}{{\bf 0}}
\newcommand{\bfone}{{\bf 1}}
\newcommand{\bftwo}{{\bf 2}}
\newcommand{\bfthree}{{\bf 3}}
\newcommand{\bffour}{{\bf 4}}
\newcommand{\bffive}{{\bf 5}}
\newcommand{\bfsix}{{\bf 6}}
\newcommand{\bfseven}{{\bf 7}}
\newcommand{\bfeight}{{\bf 8}}
\newcommand{\bfnine}{{\bf 9}}

\newcommand{\sfzero}{{\sf 0}}
\newcommand{\sfone}{{\sf 1}}
\newcommand{\sftwo}{{\sf 2}}
\newcommand{\sfthree}{{\sf 3}}
\newcommand{\sffour}{{\sf 4}}
\newcommand{\sffive}{{\sf 5}}
\newcommand{\sfsix}{{\sf 6}}
\newcommand{\sfseven}{{\sf 7}}
\newcommand{\sfeight}{{\sf 8}}
\newcommand{\sfnine}{{\sf 9}}
\newcommand{\pfzero}{\mbox{\small\pfont 0}}
\newcommand{\pfone}{\mbox{\small\pfont 1}}
\newcommand{\pftwo}{\mbox{\small\pfont 2}}
\newcommand{\pfthree}{\mbox{\small\pfont 3}}
\newcommand{\pffour}{\mbox{\small\pfont 4}}
\newcommand{\pffive}{\mbox{\small\pfont 5}}
\newcommand{\pfsix}{\mbox{\small\pfont 6}}
\newcommand{\pfseven}{\mbox{\small\pfont 7}}
\newcommand{\pfeight}{\mbox{\small\pfont 8}}
\newcommand{\pfnine}{\mbox{\small\pfont 9}}

\newcommand{\req}{\; \raisebox{0.4mm}{$\rightharpoonup$}\!\!\!\!\!\!
	\raisebox{-0.4mm}{$\rightharpoondown$} \;}  % = pointing right
%  \newcommand{\bfeq}{{\bf =}}
% \newcommand{\feq}{\hbox{$\,\thickapprox\,$}}
\newcommand{\feq}{\hbox{\boldmath $\,\doteq\,$}}
\newcommand{\notfeq}{\hbox{$\,\not\thickapprox\,$}}
\newcommand{\bfeq}{\hbox{\hspace{.2mm}\rule[1.2mm]{2mm}{.4mm}\hspace{-2mm}\rule[.2mm]{2mm}{.4mm}\hspace{.3mm}}}
\newcommand{\notbfeq}{\!\not{\!\!\bfeq}\,}
\newcommand{\bfplus}{\hbox{$\boldsymbol +$}}
\newcommand{\bftimes}{\hbox{$\boldsymbol \times$}}

\newcommand{\itA}{{\it A}}
\newcommand{\itB}{{\it B}}
\newcommand{\itC}{{\it C}}
\newcommand{\itD}{{\it D}}
\newcommand{\itE}{{\it E}}
\newcommand{\itF}{{\it F}}
\newcommand{\itG}{{\it G}}
\newcommand{\itH}{{\it H}}
\newcommand{\itI}{{\it I}}
\newcommand{\itJ}{{\it J}}
\newcommand{\itK}{{\it K}}
\newcommand{\itL}{{\it L}}
\newcommand{\itM}{{\it M}}
\newcommand{\itN}{{\it N}}
\newcommand{\itO}{{\it O}}
\newcommand{\itP}{{\it P}}
\newcommand{\itQ}{{\it Q}}
\newcommand{\itR}{{\it R}}
\newcommand{\itS}{{\it S}}
\newcommand{\itT}{{\it T}}
\newcommand{\itU}{{\it U}}
\newcommand{\itV}{{\it V}}
\newcommand{\itW}{{\it W}}
\newcommand{\itX}{{\it X}}
\newcommand{\itY}{{\it Y}}
\newcommand{\itZ}{{\it Z}}

\newcommand{\rmA}{{\rm A}}
\newcommand{\rmB}{{\rm B}}
\newcommand{\rmC}{{\rm C}}
\newcommand{\rmD}{{\rm D}}
\newcommand{\rmE}{{\rm E}}
\newcommand{\rmF}{{\rm F}}
\newcommand{\rmG}{{\rm G}}
\newcommand{\rmH}{{\rm H}}
\newcommand{\rmI}{{\rm I}}
\newcommand{\rmJ}{{\rm J}}
\newcommand{\rmK}{{\rm K}}
\newcommand{\rmL}{{\rm L}}
\newcommand{\rmM}{{\rm M}}
\newcommand{\rmN}{{\rm N}}
\newcommand{\rmO}{{\rm O}}
\newcommand{\rmP}{{\rm P}}
\newcommand{\rmQ}{{\rm Q}}
\newcommand{\rmR}{{\rm R}}
\newcommand{\rmS}{{\rm S}}
\newcommand{\rmT}{{\rm T}}
\newcommand{\rmU}{{\rm U}}
\newcommand{\rmV}{{\rm V}}
\newcommand{\rmW}{{\rm W}}
\newcommand{\rmX}{{\rm X}}
\newcommand{\rmY}{{\rm Y}}
\newcommand{\rmZ}{{\rm Z}}

\newcommand{\calA}{\hbox{$\cal A$}}
\newcommand{\calB}{\hbox{$\cal B$}}
\newcommand{\calC}{\hbox{$\cal C$}}
\newcommand{\calD}{\hbox{$\cal D$}}
\newcommand{\calE}{\hbox{$\cal E$}}
\newcommand{\calF}{\hbox{$\cal F$}}
\newcommand{\calG}{\hbox{$\cal G$}}
\newcommand{\calH}{\hbox{$\cal H$}}
\newcommand{\calI}{\hbox{$\cal I$}}
\newcommand{\calJ}{\hbox{$\cal J$}}
\newcommand{\calK}{\hbox{$\cal K$}}
\newcommand{\calL}{\hbox{$\cal L$}}
\newcommand{\calM}{\hbox{$\cal M$}}
\newcommand{\calN}{\hbox{$\cal N$}}
\newcommand{\calO}{\hbox{$\cal O$}}
\newcommand{\calP}{\hbox{$\cal P$}}
\newcommand{\calQ}{\hbox{$\cal Q$}}
\newcommand{\calR}{\hbox{$\cal R$}}
\newcommand{\calS}{\hbox{$\cal S$}}
\newcommand{\calT}{\hbox{$\cal T$}}
\newcommand{\calU}{\hbox{$\cal U$}}
\newcommand{\calV}{\hbox{$\cal V$}}
\newcommand{\calW}{\hbox{$\cal W$}}
\newcommand{\calX}{\hbox{$\cal X$}}
\newcommand{\calY}{\hbox{$\cal Y$}}
\newcommand{\calZ}{\hbox{$\cal Z$}}

\newcommand{\ttA}{\hbox{$\tt A$}}
\newcommand{\ttB}{\hbox{$\tt B$}}
\newcommand{\ttC}{\hbox{$\tt C$}}
\newcommand{\ttD}{\hbox{$\tt D$}}
\newcommand{\ttE}{\hbox{$\tt E$}}
\newcommand{\ttF}{\hbox{$\tt F$}}
\newcommand{\ttG}{\hbox{$\tt G$}}
\newcommand{\ttH}{\hbox{$\tt H$}}
\newcommand{\ttI}{\hbox{$\tt I$}}
\newcommand{\ttJ}{\hbox{$\tt J$}}
\newcommand{\ttK}{\hbox{$\tt K$}}
\newcommand{\ttL}{\hbox{$\tt L$}}
\newcommand{\ttM}{\hbox{$\tt M$}}
\newcommand{\ttN}{\hbox{$\tt N$}}
\newcommand{\ttO}{\hbox{$\tt O$}}
\newcommand{\ttP}{\hbox{$\tt P$}}
\newcommand{\ttQ}{\hbox{$\tt Q$}}
\newcommand{\ttR}{\hbox{$\tt R$}}
\newcommand{\ttS}{\hbox{$\tt S$}}
\newcommand{\ttT}{\hbox{$\tt T$}}
\newcommand{\ttU}{\hbox{$\tt U$}}
\newcommand{\ttV}{\hbox{$\tt V$}}
\newcommand{\ttW}{\hbox{$\tt W$}}
\newcommand{\ttX}{\hbox{$\tt X$}}
\newcommand{\ttY}{\hbox{$\tt Y$}}
\newcommand{\ttZ}{\hbox{$\tt Z$}}

\newcommand{\scA}{\hbox{\sc A}}
\newcommand{\scB}{\hbox{\sc B}}
\newcommand{\scC}{\hbox{\sc C}}
\newcommand{\scD}{\hbox{\sc D}}
\newcommand{\scE}{\hbox{\sc E}}
\newcommand{\scF}{\hbox{\sc F}}
\newcommand{\scG}{\hbox{\sc G}}
\newcommand{\scH}{\hbox{\sc H}}
\newcommand{\scI}{\hbox{\sc I}}
\newcommand{\scJ}{\hbox{\sc J}}
\newcommand{\scK}{\hbox{\sc K}}
\newcommand{\scL}{\hbox{\sc L}}
\newcommand{\scM}{\hbox{\sc M}}
\newcommand{\scN}{\hbox{\sc N}}
\newcommand{\scO}{\hbox{\sc O}}
\newcommand{\scP}{\hbox{\sc P}}
\newcommand{\scQ}{\hbox{\sc Q}}
\newcommand{\scR}{\hbox{\sc R}}
\newcommand{\scS}{\hbox{\sc S}}
\newcommand{\scT}{\hbox{\sc T}}
\newcommand{\scU}{\hbox{\sc U}}
\newcommand{\scV}{\hbox{\sc V}}
\newcommand{\scW}{\hbox{\sc W}}
\newcommand{\scX}{\hbox{\sc X}}
\newcommand{\scY}{\hbox{\sc Y}}
\newcommand{\scZ}{\hbox{\sc Z}}

\newcommand{\dA}{\hbox{$\Bbb A$}}
\newcommand{\dB}{\hbox{$\Bbb B$}}
\newcommand{\dC}{\hbox{$\Bbb C$}}
\newcommand{\dD}{\hbox{$\Bbb D$}}
\newcommand{\dE}{\hbox{$\Bbb E$}}
\newcommand{\dF}{\hbox{$\Bbb F$}}
\newcommand{\dG}{\hbox{$\Bbb G$}}
\newcommand{\dH}{\hbox{$\Bbb H$}}
\newcommand{\dI}{\hbox{$\Bbb I$}}
\newcommand{\dJ}{\hbox{$\Bbb J$}}
\newcommand{\dK}{\hbox{$\Bbb K$}}
\newcommand{\dL}{\hbox{$\Bbb L$}}
\newcommand{\dM}{\hbox{$\Bbb M$}}
\newcommand{\dN}{\hbox{$\Bbb N$}}
\newcommand{\dO}{\hbox{$\Bbb O$}}
\newcommand{\dP}{\hbox{$\Bbb P$}}
\newcommand{\dQ}{\hbox{$\Bbb Q$}}
\newcommand{\dR}{\hbox{$\Bbb R$}}
\newcommand{\dS}{\hbox{$\Bbb S$}}
\newcommand{\dT}{\hbox{$\Bbb T$}}
\newcommand{\dU}{\hbox{$\Bbb U$}}
\newcommand{\dV}{\hbox{$\Bbb V$}}
\newcommand{\dW}{\hbox{$\Bbb W$}}
\newcommand{\dX}{\hbox{$\Bbb X$}}
\newcommand{\dY}{\hbox{$\Bbb Y$}}
\newcommand{\dZ}{\hbox{$\Bbb Z$}}

\newcommand{\gra}{\hbox{$\alpha$}}
\newcommand{\grb}{\hbox{$\beta$}}
\newcommand{\grg}{\hbox{$\gamma$}}
\newcommand{\grd}{\hbox{$\delta$}}
\newcommand{\gre}{\hbox{$\varepsilon$}}
\newcommand{\grh}{\hbox{$\eta$}}
\newcommand{\grz}{\hbox{$\zeta$}}
\newcommand{\grth}{\hbox{$\theta$}}
\newcommand{\gri}{\hbox{$\iota$}}
\newcommand{\grk}{\hbox{$\kappa$}}
\newcommand{\grl}{\hbox{$\lambda$}}
\newcommand{\grm}{\hbox{$\mu$}}
\newcommand{\grn}{\hbox{$\nu$}}
\newcommand{\grx}{\hbox{$\xi$}}
\newcommand{\gro}{\hbox{$o$}}
\newcommand{\grp}{\hbox{$\pi$}}
\newcommand{\grr}{\hbox{$\rho$}}
\newcommand{\grs}{\hbox{$\sigma$}}
\newcommand{\grt}{\hbox{$\tau$}}
\newcommand{\gru}{\hbox{$\upsilon$}}
\newcommand{\grf}{\hbox{$\varphi$}}
\newcommand{\grch}{\hbox{$\chi$}}
\newcommand{\grq}{\hbox{$\psi$}}
\newcommand{\grw}{\hbox{$\omega$}}

\newcommand{\grG}{\hbox{$\Gamma$}}
\newcommand{\grD}{\hbox{$\Delta$}}
\newcommand{\grT}{\hbox{$\Theta$}}
\newcommand{\grTh}{\hbox{$\Theta$}}
\newcommand{\grTH}{\hbox{$\Theta$}}
\newcommand{\grL}{\hbox{$\Lambda$}}
\newcommand{\grX}{\hbox{$\Xi$}}
\newcommand{\grP}{\hbox{$\Pi$}}
\newcommand{\grS}{\hbox{$\Sigma$}}
\newcommand{\grU}{\hbox{$\Upsilon$}}
\newcommand{\grF}{\hbox{$\Phi$}}
\newcommand{\grQ}{\hbox{$\Psi$}}
\newcommand{\grW}{\hbox{$\Omega$}}

\newcommand{\igra}{\hbox{$\mit\alpha$}}
\newcommand{\igrb}{\hbox{$\mit\beta$}}
\newcommand{\igrg}{\hbox{$\mit\gamma$}}
\newcommand{\igrd}{\hbox{$\mit\delta$}}
\newcommand{\igre}{\hbox{$\mit\epsilon$}}
\newcommand{\igrh}{\hbox{$\mit\eta$}}
\newcommand{\igrz}{\hbox{$\mit\zeta$}}
\newcommand{\igrth}{\hbox{$\mit\theta$}}
\newcommand{\igri}{\hbox{$\mit\iota$}}
\newcommand{\igrk}{\hbox{$\mit\kappa$}}
\newcommand{\igrl}{\hbox{$\mit\lambda$}}
\newcommand{\igrm}{\hbox{$\mit\mu$}}
\newcommand{\igrn}{\hbox{$\mit\nu$}}
\newcommand{\igrx}{\hbox{$\mit\xi$}}
\newcommand{\igro}{\hbox{$\mit\omicron$}}
\newcommand{\igrp}{\hbox{$\mit\pi$}}
\newcommand{\igrr}{\hbox{$\mit\rho$}}
\newcommand{\igrt}{\hbox{$\mit\tau$}}
\newcommand{\igru}{\hbox{$\mit\upsilon$}}
\newcommand{\igrf}{\hbox{$\mit\varphi$}}
\newcommand{\igrch}{\hbox{$\mit\chi$}}
\newcommand{\igrq}{\hbox{$\mit\psi$}}
\newcommand{\igrw}{\hbox{$\mit\omega$}}

\newcommand{\igrG}{\hbox{$\mit\Gamma$}}
\newcommand{\igrD}{\hbox{$\mit\Delta$}}
\newcommand{\igrT}{\hbox{$\mit\Theta$}}
\newcommand{\igrL}{\hbox{$\mit\Lambda$}}
\newcommand{\igrX}{\hbox{$\mit\Xi$}}
\newcommand{\igrP}{\hbox{$\mit\Pi$}}
\newcommand{\igrS}{\hbox{$\mit\Sigma$}}
\newcommand{\igrU}{\hbox{$\mit\Upsilon$}}
\newcommand{\igrF}{\hbox{$\mit\Phi$}}
\newcommand{\igrQ}{\hbox{$\mit\Psi$}}
\newcommand{\igrW}{\hbox{$\mit\Omega$}}

\newcommand{\bgra}{\hbox{\boldmath$\alpha$}}
\newcommand{\bgrb}{\hbox{\boldmath$\beta$}}
\newcommand{\bgrg}{\hbox{\boldmath$\gamma$}}
\newcommand{\bgrd}{\hbox{\boldmath$\delta$}}
\newcommand{\bgre}{\hbox{\boldmath$\varepsilon$}}
\newcommand{\bgrz}{\hbox{\boldmath$\zeta$}}
\newcommand{\bgrh}{\hbox{\boldmath$\eta$}}
\newcommand{\bgrth}{\hbox{\boldmath$\theta$}}
\newcommand{\bgri}{\hbox{\boldmath$\iota$}}
\newcommand{\bgrk}{\hbox{\boldmath$\kappa$}}
\newcommand{\bgrl}{\hbox{\boldmath$\lambda$}}
\newcommand{\bgrm}{\hbox{\boldmath$\mu$}}
\newcommand{\bgrn}{\hbox{\boldmath$\nu$}}
\newcommand{\bgrx}{\hbox{\boldmath$\xi$}}
\newcommand{\bgro}{\hbox{\boldmath$\omicron$}}
\newcommand{\bgrp}{\hbox{\boldmath$\pi$}}
\newcommand{\bgrr}{\hbox{\boldmath$\rho$}}
\newcommand{\bgrs}{\hbox{\boldmath$\sigma$}}
\newcommand{\bgrt}{\hbox{\boldmath$\tau$}}
\newcommand{\bgru}{\hbox{\boldmath$\upsilon$}}
\newcommand{\bgrf}{\hbox{\boldmath$\varphi$}}
\newcommand{\bgrch}{\hbox{\boldmath$\chi$}}
\newcommand{\bgrq}{\hbox{\boldmath$\psi$}}
\newcommand{\bgrw}{\hbox{\boldmath$\omega$}}

\newcommand{\bgrG}{\hbox{\boldmath$\Gamma$}}
\newcommand{\bgrD}{\hbox{\boldmath$\Delta$}}
\newcommand{\bgrT}{\hbox{\boldmath$\Theta$}}
\newcommand{\bgrL}{\hbox{\boldmath$\Lambda$}}
\newcommand{\bgrX}{\hbox{\boldmath$\Xi$}}
\newcommand{\bgrP}{\hbox{\boldmath$\Pi$}}
\newcommand{\bgrS}{\hbox{\boldmath$\Sigma$}}
\newcommand{\bgrU}{\hbox{\boldmath$\Upsilon$}}
\newcommand{\bgrF}{\hbox{\boldmath$\Phi$}}
\newcommand{\bgrQ}{\hbox{\boldmath$\Psi$}}
\newcommand{\bgrW}{\hbox{\boldmath$\Omega$}}

\newcommand{\bigrG}{\hbox{\boldmath$\Gamma$}}
\newcommand{\bigrD}{\hbox{\boldmath$\Delta$}}
\newcommand{\bigrT}{\hbox{\boldmath$\Theta$}}
\newcommand{\bigrL}{\hbox{\boldmath$\Lambda$}}
\newcommand{\bigrX}{\hbox{\boldmath$\Xi$}}
\newcommand{\bigrP}{\hbox{\boldmath$\Pi$}}
\newcommand{\bigrS}{\hbox{\boldmath$\Sigma$}}
\newcommand{\bigrU}{\hbox{\boldmath$\Upsilon$}}
\newcommand{\bigrF}{\hbox{\boldmath$\Phi$}}
\newcommand{\bigrQ}{\hbox{\boldmath$\Psi$}}
\newcommand{\bigrW}{\hbox{\boldmath$\Omega$}}

\newcommand{\godel}{G\"{o}del}
\newcommand{\lob}{L\"{o}b}
\newcommand{\grze}{Grzegorczyk}
\newcommand{\bohm}{B\"{o}hm}
\newcommand{\konig}{K\"{o}nig}
\newcommand{\schutte}{Sch\"{u}tte}
\newcommand{\lowenheim}{L\"{o}wenheim}
\newcommand{\ie}{i.e.\ }
\newcommand{\eg}{e.g.\ }

%  PROGRAMS KEYWORDS
%  \input{/usr/dml/macros/programkeyword}
%  \newcommand{\strng}{{\sc string}}
\newcommand{\iif}{\hbox{ {\tt if} }}  %another form below
\newcommand{\jump}{\hbox{ {\tt jump} }}
\newcommand{\bkup}{\hbox{ {\tt bkup} }}
\newcommand{\halt}{\hbox{ {\tt halt} }}
\newcommand{\hd}{\hbox{ {\tt hd} }}
\newcommand{\tl}{\hbox{ {\tt tl} }}
\newcommand{\lst}{\hbox{ {\tt lst} }}
\newcommand{\shrt}{\hbox{ {\tt shrt} }}
\newcommand{\abort}{\hbox{ {\tt abort} }}
\newcommand{\state}{\hbox{ {\tt state} }}
%  \newcommand{\iif}{\; \underline{\rm if}\; }
%  \newcommand{\then}{\; \underline{\rm then}\; }
%  \newcommand{\goto}{\; \underline{\rm goto} \;}
%  \newcommand{\eelse}{\; \underline{\rm else}\; }

% TURING MACHINES
%  \input{/usr/dml/macros/turingmachine}
\newcommand{\leftword}{\hbox{ {\tt leftword} }}
\newcommand{\scanned}{\hbox{ {\tt scanned} }}
\newcommand{\rightword}{\hbox{ {\tt rightword} }}
\newcommand{\act}{\hbox{ {\tt act} }}

% MATHEMATICAL SYMBOLS ABBREVIATIONS
%  \input{/usr/dml/macros/mathsymbol}
%  \newcommand{\forces}{{\small \mid}\vdash}
\newcommand{\vdasheq}{\vdash\!\!\! ^{ ^=}\,}
\newcommand{\notvdasheq}{\not\vdash\!\!\! ^{ ^=}\,}
\newcommand{\forces}{\;\|\!\!\!-}
\newcommand{\force}{\;\|\!\!\!-}
\newcommand{\sbwedge}{\hbox{$\bigwedge$}} % bigwedge in line mode
\newcommand{\sbvee}{\hbox{$\bigvee$}}
\newcommand{\ra}{\rightarrow}
\newcommand{\pa}{\rightharpoonup}
\newcommand{\pra}{\rightharpoonup}	% patial function
\newcommand{\spra}{\!\rightharpoonup\!} % short partial function
\newcommand{\sra}{\!\rightarrow\!} % short rightarrow (less spaces)
\newcommand{\Sla}{\!\leftarrow\!} % short leftarrow (less spaces)
\newcommand{\slra}{\!\leftrightarrow\!}
\newcommand{\rpa}{\rightharpoonup}
\newcommand{\la}{\leftarrow}
\newcommand{\str}{\small\sf} 
\newcommand{\rra}{\rightrightarrows}  %  parallel right arrows
\newcommand{\rA}{\Rightarrow}  %  method: A= double arrow ; L/R long
\newcommand{\srA}{\!\Rightarrow\!} 
\newcommand{\lA}{\Leftarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\lrA}{\Leftrightarrow}
\newcommand{\La}{\longleftarrow}
\newcommand{\Ra}{\longrightarrow}
\newcommand{\LA}{\Longleftarrow}
\newcommand{\RA}{\Longrightarrow}
\newcommand{\LRA}{\Longleftrightarrow}
\newcommand{\LRa}{\longleftrightarrow}
\newcommand{\homom}{\stackrel{\hbox{\scriptsize\it hom}}{\longrightarrow}}  
	% homomorphism
\newcommand{\bij}{\cong}
%  \newcommand{\bij}{\rightarrow_{\hbox{\scriptsize\it bij}}}  % bijection
\newcommand{\inj}{\rightarrow_{\hbox{\scriptsize\it inj}}}  % injection
\newcommand{\srj}{\rightarrow_{\hbox{\scriptsize\it srj}}}  % surjection
%  \newcommand{\bij}{\stackrel{\hbox{\scriptsize\it bij}}{\longrightarrow}}  % bijection
%  \newcommand{\inj}{\stackrel{\hbox{\scriptsize\it inj}}{\longrightarrow}}  % injection
%  \newcommand{\srj}{\stackrel{\hbox{\scriptsize\it srj}}{\longrightarrow}}  % surjection
\newcommand{\sdot}{\!\cdot\!} % short central dot
\newcommand{\stimes}{\!\times\!}
\newcommand{\splus}{\!+\!}
\newcommand{\sminus}{\!-\!}
\newcommand{\sequal}{\!=\!}
\newcommand{\cutsubtr}{\stackrel{.}{-}}		% cut-off subtraction
\newcommand{\sgt}{\!>\!}
\newcommand{\sleq}{\!\leq\!}
\newcommand{\sgeq}{\!\geq\!}
% \newcommand{\arity}{\hbox{\it arity$\,$}}
\newcommand{\arity}{\fnc{arity}}
\newcommand{\hyphen}{\hbox{-}}
\newcommand{\degree}{\hbox{\it degree$\,$}}
\newcommand{\dom}{\hbox{\rm dom$\,$}}
\newcommand{\cod}{\hbox{\rm codom$\,$}}
\newcommand{\rnge}{\hbox{\rm rng$\,$}}
\newcommand{\Id}{\hbox{\rm Id}}
\newcommand{\Idf}{\hbox{\it Idf$\,$}}
\newcommand{\vrb}{\hbox{\it Vrb$\,$}}
\newcommand{\modd}{\hbox{\it Mod}}

\newcommand{\lbl}[1]{\hbox{\scriptsize\rm #1}}  % label for nat deductn etc


% MATHEMATICAL UTILITY SYMBOLS

%  \input{/usr/dml/macros/mathutility}

% \renewcommand{\Box}{\square}
\newcommand{\qed}{\hfill {\boldmath$\Box$}\\}
% \newcommand{\qed}{\hfill{\Large\boldmath$\dashv$}}
% \newcommand{\qed}{\hspace*{\fill}$\dashv$}
%  \newcommand{\qed}{\mx[2mm]{} $\Box$}
%  \newcommand{\qed}{\newline $\Box$}
%  \newcommand{\qed}{\newline $\spadesuit$}
\newcommand{\Qed}{\zero\hfill{\Large\boldmath$\Box$}}
\newcommand{\QED}{\zero\hfill{\Large\boldmath$\Box$}}
% \newcommand{\Qed}{\zero\hfill$\dashv$}
%  \newcommand{\Qed}{$\spadesuit$}
\newcommand{\lng}{\langle}
\newcommand{\rng}{\rangle}
\newcommand{\lft}{\hbox{\scriptsize $>$}}   % left delimiter
\newcommand{\df}{=_{\rm df}}
\newcommand{\Df}{=_{\rm df}}
\newcommand{\dfr}{\;\equiv_{\rm df}\;}
%  \newcommand{\st}{\; \hbox{\large\bf :} \;}
\newcommand{\suchthat}{\;\; \hbox{\Large\bf :} \;\;}
% \newcommand{\mod}{{\rm mod \,}}
\newcommand{\copro}{{\cal q}}
\newcommand{\mutualinterp}{\lhd \hspace{-7pt} \rhd \;}
\newcommand{\mutualembed}{\lhd \hspace{-7pt} \rhd \;}
\newcommand{\mutualsemiinterp}{\prec \hspace{-5pt} \succ}
\newcommand{\isom}{\mathrel{\mathop{=}\limits^{\normalsize\sim}}}
\newcommand{\rhds}{\rhd_s}
\newcommand{\qf}{quantifier-free}
\newcommand{\fvb}{{\hbox{\rm fvb}}}
\newcommand{\model}{\hbox{\it Mod}\,}
\newcommand{\ded}{\hbox{\it Ded}}
\newcommand{\struc}{\hbox{\it Struc}}
\newcommand{\fml}{\hbox{\it Fml}}
\newcommand{\snt}{\hbox{\it Snt}}
\newcommand{\env}{\hbox{\it Env}}
\newcommand{\semr}{]\hspace{-0.5mm}]} % semantic double bracket (right)
\newcommand{\seml}{[\hspace{-0.5mm}[} % semantic double bracket (left)
\newcommand{\rsem}{]\hspace{-0.5mm}]} % semantic double bracket (right)
\newcommand{\lsem}{[\hspace{-0.5mm}[} % semantic double bracket (left)
\newcommand{\sem}[1]{\seml #1 \semr}
%  \renewcommand{\emptyset}{\varnothing}
%  \renewcommand{\geq}{\vargeq}
%  \renewcommand{\leq}{\varleq}
%  \renewcommand{\subseteq}{\varsubseteq}
%  \renewcommand{\supseteq}{\varsupseteq}
\newcommand{\rest}{\!\upharpoonright\!}
\newcommand{\onl}{\hbox{\it Onl}}
\newcommand{\cnl}{\hbox{\it Cnl}}


% THEORIES AND SCHEMAS

%  \input{/usr/dml/macros/theory}

\newcommand{\solt}{{\bf SOL}^\Theta}
\newcommand{\il}{\bf 2\bgrl}
\newcommand{\iil}{\bf 2\bgrl}
\newcommand{\pl}{\hbox{$\bfS\bfF_2$}}
%  \newcommand{\pl}{\hbox{\bf S2\bgrl}}
%  \newcommand{\pl}{{\cal S}2\lambda}
\newcommand{\siil}{{\bf S2}\lambda}
%  \newcommand{\siil}{{\cal S}2\lambda}
\newcommand{\upl}{{\bf P2}\bgrl}
%  \newcommand{\upl}{{\cal P}2\lambda}
\newcommand{\piil}{{\bf P2}\bgrl}
%  \newcommand{\piil}{{\cal P}2\lambda}
\newcommand{\iiL}{{\bf 2}{\cal L}}
\newcommand{\siiL}{{\bf S2}{\cal L}}
%  \newcommand{\siiL}{{\cal S}2{\cal L}}
\newcommand{\piiL}{{\bf P2}{\cal L}}
%  \newcommand{\piiL}{{\cal P}2{\cal L}}

% MACROS ABBREVIATIONS

\newcommand{\ifthn}[2]{\text{ if } #1 \text{ then } #2}
\newcommand{\ifthnels}[3]{\text{ if } #1 \text{ then } #2 \text{ else } #3}
\newcommand{\ignore}[1]{}
\newenvironment{Ignore}{\ignore}{}
%  \input{/usr/dml/macros/macro}
%  \newcommand{\beq}{$$}
%  \newcommand{\eeq}{$$}
\newcommand{\Indent}{\zero\\[-\baselineskip]\indent}% indent even @ start of sec
\newcommand{\mx}{\makebox}
\newcommand{\vac}{\mx[1cm]{}}
\newcommand{\zero}{\rule{0mm}{3mm}}
\newcommand{\halfmm}{\mx[0.5mm]{}}
\newcommand{\onemm}{\mx[1mm]{}}
\newcommand{\minusonemm}{\mx[-1mm]{}}
\newcommand{\minustwomm}{\mx[-2mm]{}}
\newcommand{\twomm}{\mx[2mm]{}}
\newcommand{\threemm}{\mx[3mm]{}}
\newcommand{\fourmm}{\mx[4mm]{}}
\newcommand{\fivemm}{\mx[5mm]{}}
\newcommand{\sixmm}{\mx[6mm]{}}
\newcommand{\sevenmm}{\mx[7mm]{}}
\newcommand{\eightmm}{\mx[8mm]{}}
\newcommand{\ninemm}{\mx[9mm]{}}
\newcommand{\onecm}{\mx[1cm]{}}
\newcommand{\twocm}{\mx[2cm]{}}
\newcommand{\threecm}{\mx[3cm]{}}
\newcommand{\fourcm}{\mx[4cm]{}}
\newcommand{\fivecm}{\mx[5cm]{}}
\newcommand{\sixcm}{\mx[6cm]{}}
\newcommand{\sevencm}{\mx[7cm]{}}
\newcommand{\eightcm}{\mx[8cm]{}}
\newcommand{\ninecm}{\mx[9cm]{}}
\newcommand{\tencm}{\mx[10cm]{}}
\newcommand{\back}{\!\!}
\newcommand{\sepline}{\bigskip\noindent\rule{0mm}{1mm}\hrulefill\rule{0mm}{1mm}\bigskip}		% in-text separation line 
\newcommand{\next}{\newline \zero \qquad}
\newcommand{\nextt}{\\ \zero\qquad}
\newcommand{\nexttt}{\\ \zero\quad\quad}
\newcommand{\nnext}{\newline \zero \qquad\qquad}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\itemm}{\item\zero}
\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\bd}{\begin{description}}
\newcommand{\ed}{\end{description}}
\newcommand{\beqn}{\begin{equation}}
\newcommand{\eeqn}{\end{equation}}
\newcommand{\beqns}{\begin{equation\*}}
\newcommand{\eeqns}{\end{equation\*}}
\newcommand{\beqna}{\begin{eqnarray}}
\newcommand{\eeqna}{\end{eqnarray}}
\newcommand{\beqnas}{\begin{eqnarray*}}
\newcommand{\eeqnas}{\end{eqnarray*}}
\newcommand{\beqnaa}{$$\begin{array}{rcll}}  %  begin annotated eqn array
\newcommand{\eeqnaa}{\end{array}$$}  %  end annotated eqn array
\newcommand{\beqnana}{$$\begin{array}{lrcll}}  % eqn array numbrd & annttd 
\newcommand{\eeqnana}{\end{array}$$}  %  end annotated eqn array
\newcommand{\btbl}[1]{\begin{center}\begin{tabular}{#1}}
\newcommand{\etbl}{\end{tabular}\end{center}}
\newcommand{\beqnc}{$$\begin{array}{rclcl}}
\newcommand{\eeqnc}{\end{array}$$}
\newcommand{\fn}{\footnote}
\newcommand{\credit}[1]{{\normalsize [#1]}}
\newcommand{\head}[1]{\noindent{\LARGE\bf #1} \\ \medskip}

%  ENVIRONMENTS

%  \input{/usr/dml/macros/environment}
\newenvironment{comment}{\begin{quote}\small}{\end{quote}}
%  \newenvironment{comment}{\addtolength{\leftmargini}{+1in}\small}{\addtolength{\leftmargini}{-1in}\normalsize}

\newcommand{\Section}[1]{\newpage {\Large \section{#1}}}
\newcommand{\Sectionnonumber}[1]{\newpage {\Large \section*{#1}}}
\newcommand{\Sectionsamepage}[1]{\vspace{5mm}{\Large \section{#1}}}
\newcommand{\Sectionsamepagenonumber}[1]{\vspace{5mm}{\Large \section*{#1}}}
\newcommand{\Sectionnonumbersamepage}[1]{{\Large \section*{#1}}}
\newcommand{\Sectionn}[1]{{\Large \section*{#1}}}
\newcommand{\Subsection}[1]{\bigskip{\large \subsection{#1}}}
\newcommand{\Ssubsection}[2]{\bigskip{\large \subsection{#1}\label{#2}}}

\newcommand{\parag}[1]{\medskip \noindent {\large\sf {#1}} \onecm}
\newcommand{\Prop}[1]{\begin{prop}{\rm #1}\end{prop}}
% \newcommand{\proof}{{\bf Proof. }}
\newcommand{\prf}{{\sc Proof. }}
\newcommand{\prfof}[1]{{\bf \zero\\ Proof of {#1}. }}
\newcommand{\prfsktch}{{\bf Proof sketch. }}
\newcommand{\prfsketch}{{\bf Proof sketch. }}
\newcommand{\prfoutline}{{\bf Proof outline. }}
\newcommand{\prfidea}{{\bf Proof Idea. }}

%  option 1:  
%  theorems numbered in roman, other theorem-like environments nmbrd separately
\newtheorem{dclprop}{{\sc Proposition}} % prop's # regardless of sections
% \newtheorem{dclprop}{{\sc Proposition}}[section] % prop's subnumber section
\newtheorem{dclprops}{{\sc Proposition}}[subsection] % prp's subnmbr subsection
\newtheorem{dclbigthm}[dclprop]{THEOREM}
\renewcommand{\thedclbigthm}{\Roman{dclbigthm}}
\makeatletter
\def\thmlabel#1{\@bsphack\if@filesw {\let\thepage\relax
\xdef\@gtempa{\write\@auxout{\string
\newlabel{#1}{{\@Roman{\@currentlabel}}{\thepage}}}}}\@gtempa
\if@nobreak \ifvmode\nobreak\fi\fi\fi\@esphack}
\makeatother

% option 2:
%  theorems like other theorem-like environment
\newtheorem{dclthm}[dclprop]{{\sc Theorem}}   % declare-thm environment. 
					%  thm environment defined below, 
					%  using slant font
\newtheorem{dclthms}[dclprops]{{\sc Theorem}}   % declare-thm environment,
					% numbered by subsection 

\newtheorem{dcllem}[dclprop]{{\sc Lemma}}
\newtheorem{dcllems}[dclprops]{{\sc Lemma}} % numbered by subsection
\newtheorem{dclsublem}[dclprop]{{\sc Sublemma}}
\newtheorem{dclcor}[dclprop]{{\sc Corollary}}
\newtheorem{dclcors}[dclprops]{{\sc Corollary}} % numbered by subsection
\newtheorem{dcldfn}[dclprop]{{\sc Definition}}
\newtheorem{dcldfns}[dclprops]{{\sc Definition}}% numbered by subsection
\newtheorem{dclasss}[dclprops]{{\bf Assumption}}
\newtheorem{dclass}[dclprop]{{\bf Assumption}}% numbered by subsection

\newenvironment{prop}{\medskip\begin{dclprop}\sl}{\end{dclprop}}
\newenvironment{props}{\medskip\begin{dclprops}\sl}{\end{dclprops}}
\newenvironment{thm}{\medskip\begin{dclthm}\sl}{\end{dclthm}}
% \newenvironment{thm}{\begin{dclthm}\sl}{\end{dclthm}}
\newenvironment{thms}{\medskip\begin{dclthms}\sl}{\end{dclthms}}
\newenvironment{bigthm}{\medskip\begin{dclbigthm}\sl}{\end{dclbigthm}}
\newenvironment{cors}{\medskip\begin{dclcors}\sl}{\end{dclcors}}
\newenvironment{cor}{\medskip\begin{dclcor}\sl}{\end{dclcor}}
\newenvironment{dfns}{\medskip\begin{dcldfns}\sl}{\end{dcldfns}}
\newenvironment{dfn}{\medskip\begin{dcldfn}\sl}{\end{dcldfn}}
\newenvironment{asss}{\medskip\begin{dclasss}\sl}{\end{dclasss}}
\newenvironment{ass}{\medskip\begin{dclass}\sl}{\end{dclass}}
\newenvironment{lem}{\medskip\begin{dcllem}\sl}{\end{dcllem}}
\newenvironment{lems}{\medskip\begin{dcllems}\sl}{\end{dcllems}}
\newenvironment{sublem}{\medskip\begin{dclsublem}\sl}{\end{dclsublem}}
\newenvironment{sublems}{\medskip\begin{dclsublems}\sl}{\end{dclsublems}}

\newcommand{\bsl}{\begin{verse}\sl}
\newcommand{\esl}{\end{verse}}

\newtheorem{exs}[dclprop]{Examples}
\newtheorem{ex}[dclprop]{Example}
\newenvironment{examples}{\begin{exs}\rm\bi\item[]}{\ei\end{exs}}
% \newenvironment{example}{\begin{ex}\rm}{\end{ex}}
\newtheorem{exxs}[dclprop]{Exercises}
\newtheorem{exx}[dclprop]{Exercise}

\newenvironment{exercises}{\begin{exxs}\rm\be}{\ee\end{exxs}}
\newenvironment{exercises-with-preamble}{\begin{exxs}\rm}{\end{exxs}}
\newenvironment{exwp}{\begin{exxs}\rm}{\end{exxs}}
% \newenvironment{exercise}{\begin{exx}\rm}{\end{exx}}
\newtheorem{claim}[dclprop]{Claim}
\newtheorem{comments}[dclprop]{Comments}
% \newtheorem{conj}[dclprop]{Conjuecture}

\newcommand{\bthm}{\begin{thm}}
\newcommand{\ethm}{\end{thm}}
\newcommand{\bprop}{\begin{prop}}
\newcommand{\eprop}{\end{prop}}
\newcommand{\blem}{\begin{lem}}
\newcommand{\elem}{\end{lem}}
\newcommand{\bcor}{\begin{cor}}
\newcommand{\ecor}{\end{cor}}
\newcommand{\bdfn}{\begin{dfn}}
\newcommand{\edfn}{\end{dfn}}

%  theorems numbered with other theorem-like environments
%  \newtheorem{thm}{Theorem}[section]
%  \newtheorem{prop}[thm]{Proposition}
%  \newtheorem{lem}[thm]{Lemma}
%  \newtheorem{cor}[thm]{Corollary}
%  \newtheorem{dfn}[thm]{Definition}
%  \newtheorem{ass}[thm]{Assumption}
%  \newtheorem{exs}[thm]{Examples}
%  \newtheorem{ex}[thm]{Example}
% \newenvironment{examples}{\begin{exs}\rm\be}{\ee\end{exs}}
%  \newenvironment{example}{\begin{ex}\rm}{\end{ex}}
%  \newtheorem{exxs}[thm]{Exercises}
%  \newtheorem{exx}[thm]{Exercise}
%  \newenvironment{exercises}{\begin{exxs}\rm\be}{\ee\end{exxs}}
%  \newenvironment{exerciseswithpreamble}{\begin{exxs}\rm}{\end{exxs}}
%  \newenvironment{exwp}{\begin{exxs}\rm}{\end{exxs}}
%  \newenvironment{exercise}{\begin{exx}\rm}{\end{exx}}
%  \newtheorem{claim}[thm]{Claim}
%  \newtheorem{comments}[thm]{Comments}
%  \newtheorem{conj}[thm]{Conjuecture}
%  \newenvironment{more}{\begin{quote}\small}{\end{quote}}
\newcommand{\bz}{\begin{quote}\small}
\newcommand{\ez}{\end{quote}}

% SPECIAL STRUCTURES

%  \input{/usr/dml/macros/structure}
\newcommand{\sss}{{|{\cal S}|}}
\newcommand{\turing}{{\cal T} \hspace{-3pt} uring}
\newcommand{\dstack}{{\cal D} \hspace{-3pt} stack}
\newcommand{\sd}{{\cal S} \oplus \dstack}
\newcommand{\sw}{{\cal S} \oplus {\cal W}}
%  \newcommand{\lst}{{\cal L} \hspace{-3pt} ist}
\newcommand{\tape}{{\cal T} \hspace{-3pt} ape}
%  \newcommand{\strng}{{\cal S} \hspace{-2pt} tring}
\newcommand{\term}{{\cal T} \hspace{-2pt} erm}

% SPECIAL TERMS

%  \input{/usr/dml/macros/term}
\newcommand{\mf}{mvf\ }
\newcommand{\mfs}{mvfs\ }
\newcommand{\mfp}{mvf}
\newcommand{\mfsp}{mvfs}

%  INFERENCE MACROS  for more macros and examples
%	 cf the Lechenadec file in /usr/dml/forms

%  \newcommand{\inference}[2]
  %  {\raisebox{-2mm}{\shortstack
      %  {$ #1 $\\ \mbox{}\hrulefill \mbox{}\\ $ #2 $}}}
\newcommand{\inference}[2]
  {\shortstack
      {$ #1 $\\ \mbox{}\hrulefill \mbox{}\\ $ #2 $}}
\newcommand{\einference}[2]  % "empty" (no line) inference
  {\shortstack
      {$ #1 $\\ \mbox{}\\ $ #2 $}}
% labeled inference, the label (arg. 3) should be approx. a single letter.
\newcommand{\linference}[3]
 {\raisebox{-2mm}{\shortstack{\mbox{}\\ \raisebox{1mm}{$ #3\;$} \\ \mbox{}}
  \shortstack{$ #1 $\\ \mbox{}\hrulefill \mbox{}\\ $ #2 $}}}
%  Small inferences (scriptsize)
\newcommand{\sinference}[2]
  {\shortstack
      {$\scriptstyle #1 $\\ \mbox{}\hrulefill \mbox{}\\ $\scriptstyle #2 $}}
\newcommand{\slinference}[3]
 {\shortstack{\mbox{}\\ \raisebox{1mm}{$\scriptstyle #3\;$} \\ \mbox{}}
  \shortstack{$\scriptstyle #1 $\\ \mbox{}\hrulefill 
		\mbox{}\\ $\scriptstyle #2 $}}

\newcommand{\nsections}[1]{\setcounter{subsection}{0}\setcounter{subsubsection}{0}\addtocounter{section}{1} 
	\onecm\newline\medskip\noindent{\Large\bf #1}}
\newcommand{\nsection}[1]{\setcounter{subsection}{0}\setcounter{subsubsection}{0}\addtocounter{section}{1} 
	\onecm\newline\onecm\newline\bigskip\noindent{\Large\bf \arabic{section} \ #1}}
%
\newcommand{\isection}[1]{\setcounter{subsection}{0}\setcounter{subsubsection}{0}\addtocounter{section}{1} 
	\onecm\newline\onecm\newline\noindent{\Large\bf \arabic{section} \ #1}}
\newcommand{\isectiontop}[1]{\setcounter{subsection}{0}\setcounter{subsubsection}{0}\addtocounter{section}{1} 
		\noindent{\Large\bf \arabic{section} \ #1}}
%
\newcommand{\isections}[1]{\setcounter{subsection}{0}\setcounter{subsubsection}{0}\onecm\newline\onecm\newline\bigskip\noindent{\large\bf \ #1}}
%
% following isection etc are for ieee format
% \newcommand{\nsection}[1]{\setcounter{subsection}{0}\setcounter{subsubsection}{0}\addtocounter{section}{1} 
% 	\onecm\newline\onecm\newline\bigskip\noindent{\pfont \arabic{section} \ #1}}
\newcommand{\nsubsections}[1]{\setcounter{subsubsection}{0}\addtocounter{subsection}{1} \smallskip\bigskip\noindent{\large\bf #1}\medskip}
\newcommand{\nsubsection}[1]{\setcounter{subsubsection}{0}\addtocounter{subsection}{1} \smallskip\bigskip\noindent{\large\bf \arabic{section}.\arabic{subsection} \ #1}\medskip}
\newcommand{\isubsection}[1]{\setcounter{subsubsection}{0}\addtocounter{subsection}{1} \smallskip\bigskip\noindent{\fontsize{11}{11.5}\selectfont\bf\arabic{section}.\arabic{subsection} \ #1}\medskip}
% \newcommand{\nsubsection}[1]{\setcounter{subsubsection}{0}\addtocounter{subsection}{1} \smallskip\bigskip\noindent{\large\bf \arabic{section}.\arabic{subsection} \ #1}\medskip}
\newcommand{\nfirstsubsection}[1]{\setcounter{subsubsection}{0}\addtocounter{subsection}{1} \smallskip\noindent{\large\bf \arabic{section}.\arabic{subsection} \ #1}\medskip}

% FRACTIONS IN TEX:  
%		{a}\over{b}  gives  a/b  (fraction)
%		{a}\atop{b}  gives   a above b  (like in binomial coefficient
%		{a}\above2pt{b}  gives   a/b  withj a 2pt thick fractional line


% \DeclareMathSymbol\mho     {\mathord}{lasy}{"30}
  % \DeclareMathSymbol\Join    {\mathrel}{lasy}{"31}
  % \DeclareMathSymbol\Box     {\mathord}{lasy}{"32}
  % \DeclareMathSymbol\Diamond {\mathord}{lasy}{"33}
  % \DeclareMathSymbol\leadsto {\mathrel}{lasy}{"3B}
  % \DeclareMathSymbol\sqsubset{\mathrel}{lasy}{"3C}
  % \DeclareMathSymbol\sqsupset{\mathrel}{lasy}{"3D}
  % \DeclareMathSymbol\lhd     {\mathbin}{lasy}{"01}
  % \DeclareMathSymbol\unlhd   {\mathbin}{lasy}{"02}
  % \DeclareMathSymbol\rhd     {\mathbin}{lasy}{"03}
  % \DeclareMathSymbol\unrhd   {\mathbin}{lasy}{"04}

\newcommand{\ffff}{\mbox{\sf f\hspace{-0.2mm}f}}
\newcommand{\tttt}{\mbox{\sf t\hspace{-0.3mm}t}}
% \newcommand{\ffff}{\mbox{\sf f$\!$f}}
% \newcommand{\tttt}{\mbox{\sf t$\!$t}}

% following \crossout{text} yields <text> w horizontal line through it
\newlength{\txtlth}
\newlength{\txtht}
\newcommand{\crossout}[1]
        {\settowidth{\txtlth}{#1}
         \settoheight{\txtht}{#1}
         #1\hspace{-\txtlth}\hspace{-1mm}
         \rule[\txtht/4]{\txtlth+.5mm}{.2mm}}




